Packing Compact Subgraphs with Applications to Districting

Packing disjoint subgraphs in a given graph is a fundamental problem with many applications. Motivated by political districting, we focus on connected subgraphs that are compact (e.g., having constant radius from a single center vertex) and that satisfy additional composition requirements, such as a minimum population/weight threshold or balanced weight types (e.g., political affiliations). We aim to maximize coverage by disjoint districts that meet these requirements. In this work, we present new results that substantially improve the previously known bounds on balanced star districts for planar and minor-free graphs (Dharangutte et al. 2025). In particular, we improve the approximation factor from $O(\log n)$ to $O(1)$ for packing balanced star districts using the exact same algorithm, but with a refined analysis. We also extend the results beyond planar graphs to minor-free graphs and an even broader family of graphs of bounded expansion. Additionally, we obtain an $O(1)$ approximation for packing radius-$k$ districts (with a constant $k$) in planar and apex-minor-free graphs. In order to get a $(1+\varepsilon)$ approximation on the max coverage, we show that this can be achieved if we allow a slight relaxation of the balancedness parameters (by a factor that can be made arbitrarily close to $1$), for bounded radius-$k$ districts on planar and apex-minor-free graphs. We show that all of these results can also be obtained if we enforce a minimum weight threshold for each district as the composition requirement, rather than balancedness. We present various results on hardness and hardness of approximation for this variant, by graph and district types.

==> sections/districting-problems.tex <==
\section{Solving LP and Separation Oracles}\label{sec:districting}

This section is devoted to the discussion of how to solve the LP as formulated in Section~\ref{sec:LP}. Solving the LP for $c$-balanced star districts has been discussed in prior work~\cite{Dharangutte2025-ry}. This section discusses the other variants when we consider radius $k$ or diameter $k$ for higher values of $k$ as well as the weight threshold constraint.

\subsection{Candidate Districts Are Given}\label{subsec:candidate}
\fang{small number or large number}\jie{not sure what this means}
In this setting, we assume that a set of $h$ candidate districts $\mathcal{S}=\{S_1, S_2, \cdots, S_h\}$ are given. $h$ is assumed to be polynomial of $n$. The goal is to choose a subset of disjoint districts in $\mathcal{S}$ with maximum total weight and that each district meets the properties of connectivity, compactness and additional properties of weight threshold or balancedness. 

When a polynomial number of candidate districts is specified by the problem input, we can directly apply our framework to solve for an approximate districting solution. Specifically, we first solve the LP relaxation where a candidate district can be partially chosen. Next, we round the fractional solution to an integer solution, which leads to a potential multiplicative
factor loss on the solution weight.  
This works with all versions of compactness definition (diameter or radius) and in either strong or weak notion. It also works with either or both of balanced property and weight threshold condition.

For each given candidate district $S\in \mathcal{S}$, we define a variable $x_S$ indicating whether or not this district is chosen. $x_S\in \{0, 1\}$. The integer program is exactly as defined in Equation~\ref{eq:lp-main}.
We then solve the LP program and then use randomized rounding as explained in Section~\ref{sec:LP} to derive an integer solution. 

\subsection{Candidate Districts are not Given}

In the remaining versions, we assume that the candidate districts are not given. There can be an exponential number of potential candidate districts even if parameter $k$ for compactness is a small constant. In addition, certain combinations of the requirements on candidate districts may immediately lead to NP-hard problems. For example, finding even one valid district with diameter-$1$ and a minimum weight threshold is equivalent to maximum clique problem, which is NP-hard to approximate for any factor less than $n$. 
%\jie{prathamesh, can you add hardness for general $k$ here?} 
%Even for radius $1$ (i.e., star districts), finding an optimal districting solution for $c$-balanced districts are NP-hard even for very special graphs such as complete graphs and are hard to approximate for general graphs. See~\cite{Dharangutte2025-ry} for more details.

In general, for the LP problem one cannot explicitly write down all the variables and constraints since there are exponentially many candidate districts. To address this issue we adopt the Whack-a-Mole framework \cite[Figure 3]{BKS23-lp} on the dual linear program. \shangen{I think we might want to discuss about the ellipsoid algorithm here.}\jie{can you add some?} For that, we need a \emph{separation oracle}. Specifically, we consider the dual LP problem and find a \emph{strongly violating dual constraint}, which is a district $S$ such that $\sum_{v\in S} y'_v < (1-\epsilon)\cdot w(S)$. A separation oracle either locates a good enough violating constraint or reports that all constraints are not strongly violating.
Intuitively, if all the constraints are not strongly violating, it implies that the currently maintained dual solution $\{y'_v\}$ is an $(1-\epsilon)$-approximate solution.

We formulate the task of implementing a separation oracle as follows:

\begin{mdframed}
\textbf{Input:}
Graph $G$. Dual variables $\{y'_v\}$. Weights per vertex $\{w_v\}$. An implicit set $\mathcal{S}$ of all valid districts.
\\
\textbf{Goal:} Either returns a violating district $S \in \mathcal{S}$ such that 
\begin{equation}\label{eq:violating-district}
    \sum_{v\in S} y'_v < (1-\epsilon/2) w(S); 
\end{equation}
    or reports that \emph{all} districts $S\in \mathcal{S}$ satisfy $\sum_{v \in S} y'_v \ge (1-\epsilon) w(S)$.
\end{mdframed}

In the remaining of this section we discuss which variants of the problem can be solved and how as well as hardness results for others.

% Let us define the set of all \emph{strongly violating cosntraints} as follows.
% \begin{equation}\label{eq:violate}
% \mathcal{S}_{\mathrm{violate}} := \left\{ S\ \bigg|\ \sum_{v\in S} y'_v < (1-\epsilon)\cdot w(S) \right\}.
% \end{equation}
% Our separation oracle does the following: it either returns any (possibly weaker) violating $S'$ such that 
% \begin{equation}\label{eq:weak-violate}
% \begin{aligned} 
% v\in S' && \text{and}\ \ \ \sum_{v\in S'} y'_v < (1-\epsilon/2)\cdot w(S') && \text{and}\ \ \  w(S') \ge \frac12\cdot \max_{T\in \mathcal{S}_{\mathrm{violate}}} w(T),
% \end{aligned}
% \end{equation}
% or certifies that $\mathcal{S}_\mathrm{violate}=\emptyset$.
% \jie{part of this is copied from the previous paper, which is bad. We need to rewrite it a bit.}







\subsubsection{Weight Threshold and Diameter $k$}

We show that finding just one district with weight threshold and diameter $k$ constraint is NP-hard. The formal problem definition is as follows. 

\begin{mdframed}
\textbf{Input:}
$G = (V,E)$,  weight $w_v \geq 0$ for all $v\in V$, integers $B$ and $k$. %An implicit set $\mathcal{S}$ of all valid districts such that for each $S \in \mathcal{S}$, $\text{diam}(G[S]) \leq k$.
\\
\textbf{Output:} A vertex subset $S$ such that $G[S]$ is connected,
\[
\text{diam}(G[S]) \leq k \quad \text{and} \quad w(S) := \sum_{v\in S} w_v \geq B 
\]
\end{mdframed}


\begin{theorem}
\label{thm:hardness-diam-single}
    Given a graph $G$ with integer weights $w_v \geq 0$ on vertices, integers $B > 0$ and $k \geq 1$ the problem of finding a vertex subset $S$ such that $G[S]$ is connected, diam$(G[S]) \leq k$ (strong diameter) and $w(S) \geq B$ (we call this a valid district) is NP-hard. Moreover, the problem remains NP-hard if instead we require the weak diameter of $G[S] \leq k$.
\end{theorem}

\begin{proof}
    Note that for $k = 1$, the problem reduces to finding a clique (which is hard) so we focus on $k \geq 2$. We first consider the case of strong diameter and fixed $k=2$ and show reduction form decision version of clique problem. Recall for the clique problem, given a graph $G$ and integer $T$ deciding if there is a clique of size $\geq T$ is NP-hard. 
    
    Given $G = (V,E)$ and $T$, we construct the instance $G' = (V',E')$ for the weight threshold problem as follows. For each $v \in V$, create a corresponding vertex $v' \in V'$ with $w_{v'} = 1$. For each edge $(u,v) \in E$, create a vertex $x_{(u,v)}$ with $w_{x_{(u,v)}} = 0$ and add edges $(u',x_{(u,v)})$ and $(v',x_{(u,v)})$. Add edges between all $x_{(u,v)}$ vertices in $G'$ (make it a clique).  Set $B = T$, the weight threshold for district. Observe that for any $(u,v) \in E$, distance between $u'$ and $v'$ in $G'$ is 2 (through $x_{u,v}$)and for any non-edge $(u,w)$ in $G$, distance between $u'$ and $w'$ is at least 4 (distance is 4 iff there exists $(u,q) \in E$ and $(q,w) \in E$ for some $q \in V$). 
    Now, a for a clique $S$ in $G$, $S' = \{ v' | v \in S\} \cup \{x_{(u,v)} | u \in S \;\text{and}\; v\in S\}$ forms a valid district for $k=2$ with $w(S') = |S|$. 
    This is because, $G'[S']$ is connected, pairwise distance of all vertices corresponding to clique vertices is at most 2, distance of $u'$ and $x_{(u,v)}$ for $u$ and $v$ in $S$ is at most 2 and all $x_{(u,v)}$ vertices have edges between them. Now for the other direction let $S'$ be any valid district for $k=2$ and $B = T$ in $G'$. Ignoring all the $x_{(u,v)}$ vertices in $S'$, the remaining vertices correspond to a clique in $G$ of size at least $T$. This is again because for vertices in $G'$ corresponding to vertices in $G$, distance is at most 2 iff there is an edge connecting them in $G$, and only these vertices have non-zero weight in $G'$. This completes the proof for $k=2$.

    For $k\geq3$, we describe the changes to the instance $G'$ starting with $G$, but  the core argument remains the same. For each vertex $v \in V$, create a vertex $v' \in V'$ with $w_{v'} = 1$. For each edge $(u,v) \in E$, create a vertex $x_{(u,v)}$ with $w_{x_{(u,v)}} = 0$ and create a center vertex $c$ with $w_c = 0$. Connect vertices $u'$ and $v'$ to vertex $x_{(u,v)}$ by (distinct) paths of length $\lceil k/3\rceil$, and assign weight 0 to all the nodes on the path. For all $x_{(u,v)}$ vertices, connect them with (distinct) paths of length $\lfloor k/3\rfloor$ to $c$ and assign weight 0 to all vertices on the path. Set $B = T$, the weight threshold for district. Observe, for all $(u,v) \in E$, distance between $u'$ and $v'$ in $G'$ is $\leq k$. Distance between some $v'$ and all $x_{(u,v)}$ vertices and distance between all $x_{(u,v)}$ vertices themselves is $\leq k$, through $c$. The distance for non-edge in $G$ is $> k$. The proof follows from the same argument as before.

    Now, observe that same instance and argument also hold for the case when weak diameter is restricted to be at most $k$. This is because, for a clique in $G$, we have a valid district in $G'$ with strong diameter at most $k$, which implies a valid district for weak diameter at most $k$. Also, for any connected valid district of weak diameter at most $k$ and weight $ \geq T$, the vertices with non-zero weights correspond to a clique of size $\geq T$ in $G$.
\end{proof}



Observe that the hardness of finding just one district implies the hardness for separation oracle on general graphs. This is because separation oracle requires reporting a violating constraint, which is a valid district but with small values of sum of dual variables. For $y_v = 0$ for all $v$, the same reduction above gives us the hardness result.

% \begin{theorem}
%     The problem of finding a violating district with weight threshold $B$ and diameter at most $k$ is NP-hard, for both the cases when we consider strong and weak diameter. 
% \end{theorem}
% \begin{proof}
%     We first consider the case of strong diameter and describe a reduction from the $k$-club problem on graph $G=(V,E)$. A $k$-club is a subset of vertices $S$ such that $S$ induces a graph of diameter at most $k$. The decision version of $k$-club problem is to decide if there is a $k$-club of size at least $T$ in $G$ and is NP-complete. The instance for separation oracle is as follows. Set the vertices and edges in the new instance $G' = (V',E')$ to be the same as the instance $G = (V,E)$, let $B=T$ and $\epsilon \in (0,1)$. Set $w_v = 1$ and $y_v = 0$ for all $v \in V$. Now, if $G$ has a $k$-club $S$ with $|S| \geq T$, then $S$ is a violating district in $G'$ because $S$ has diameter at most $k$ and
%     \[
%     w(S) = \sum_{v' \in S} w_v' = \sum_{v' \in S} 1 \geq B \qquad \text{and} \qquad \sum_{v' \in S} y_{v'} = 0 \leq (1 - \epsilon/2) w(S).
%     \]    
%      Similarly, if we can find a violating constraint $S'$ in $G'$ of weight at least $B$ and diameter at most $k$, these set of vertices form a $k$-club of size at least $T$ in $G$ as $w(S') = |S'| \geq T$.
% \end{proof}



As a result, we instead consider districts with bounded radius instead of diameter. Note that finding one district with bounded radius is easy - treating each vertex as a potential center, add vertices within the $k$-hop neighborhood till you exceed the weight threshold. In the following sections, we discuss the implementation of the separation oracle for bounded radius setting.


\subsubsection{Weight Threshold with Weak Radius-$k$}\label{subsec:weight-weak-radius}

To look for a candidate district that strongly violates the dual constraints, we enumerate all vertices as potential centers and consider the $k$ hop neighborhood $N_k(v)$, for each $v\in V$. Now fix a vertex $v$ and $N_k(v)$. Each node $u$ has a dual variable $y'_u
\in [0, 1]$. Thus, we would like to find a connected district within $N_k(v)$ that satisfies \Cref{eq:violating-district}. We achieve this by running an algorithm to find a `connected knapsack'. 

In a standard knapsack problem we are given a bag of capacity $W$ and candidate $n$ items where item $i$ has utility $u_i$ and weight $w_i$. The goal is to find a subset of items with total weight at most $W$ and maximum utility. In a connected knapsack problem, the items are vertices in a graph $G$ and the selected items must form a connected subgraph in $G$.

We will adapt the algorithm in~\cite{Dey2024-jg} which solves the connected knapsack problem for graphs of bounded treewidth. Specifically, we consider the value $y'_u$ to be the `weight' of $u$ and the weight $w(u)$ to be its `utility'. There are a few general remarks. First, we include node $v$ by default in the district. Second, to find a violating district $S'$, we want the total weight of the district, $w(S')$, to be at least $B$ and we would like the sum of $y$ value to be at most $(1-\epsilon/2) \cdot w(S')$. This is a variant of the knapsack problem -- fixing a minimum utility threshold and minimizing the total weight.
Second, such a connected knapsack solution will surely have weak radius $k$ since all vertices are within $N_k(v)$.

\subsubsection{Weight Threshold with Strong Radius-$2$}\label{subsec:threshold-radius-2}

We can adapt the solution in \Cref{subsec:weight-weak-radius} for the separation oracle for districts with weight threshold condition and strong radius of $1$ or $2$. For a strong radius of $1$, we are looking for star subgraphs. This can be done by using the same algorithm in \Cref{subsec:weight-weak-radius} with $k=1$. For a strong radius of $2$, we take a 2-hop neighborhood $N_2(v)$ for each potential center node $v$, and remove all edges between vertices that are exactly two hops away from $v$. We call the resulted subgraph by $N'_2(v)$. Then we apply the same algorithm in \Cref{subsec:weight-weak-radius}. Notice that in any connected district $S$ returned in $N'_2(v)$ a vertex $u$ that is $2$-hops away from $v$ must have at least one neighbor as a one-hop neighbor of $v$. Thus $S$ is an induced subgraph with radius $2$ from $v$. 


Last we remark that we do not know how to handle strong radius $k$ with $k\geq 3$. This is left as an open question. \jie{do we have anything to say about this?}

%\subsubsection{$c$-balanced District with Strong Radius-$2$}\label{subsec:balanced-radius-2}

%\begin{theorem}
%\shangen{I am not sure if this is correct yet. Po-Yu and I discussed a bit and we realize that there is no easy reduction for the separation oracle to find a diameter 2 subgraph. (One such potential missing case is the Peterson graph.)}
% Let $G$ be a graph of diameter 2. Then, there exists a connected subgraph $H$ of $O(1)$ vertices such that $V(H)$ is a dominating set of $G$.    
%\end{theorem}

%\subsubsection{$c$-balanced District with Strong Radius-$3$}\label{subsec:balanced-radius-3}




